The MAVERIC Survey: Variable Jet-Accretion Coupling in Luminous Accreting Neutron Stars in Galactic Globular Clusters

Accreting neutron stars in low-mass X-ray binaries show outflows -- and sometimes jets -- in the general manner of accreting black holes. However, the quantitative link between the accretion flow (traced by X-rays) and outflows and/or jets (traced by radio emission) is much less well-understood for neutron stars than for black holes, other than the general observation that neutron stars are fainter in the radio at a given X-ray luminosity. We use data from the deep MAVERIC radio continuum survey of Galactic globular clusters for a systematic radio and X-ray study of six luminous (L_X > 10^34 erg/s) persistent neutron star X-ray binaries in our survey, as well as two other transient systems also captured by our data. We find that these neutron star X-ray binaries show an even larger range in radio luminosity than previously observed. In particular, in quiescence at L_X ~ 3x10^34 erg/s, the confirmed neutron star binary GRS 1747--312 in Terzan 6 sits near the upper envelope of the black hole radio/X-ray correlation, and the persistently accreting neutron star systems AC 211 (in M15) and X1850--087 (in NGC 6712) show unusual radio variability and luminous radio emission. We interpret AC 211 as an obscured "Z source" that is accreting at close to the Eddington limit, while the properties of X1850--087 are difficult to explain, and motivate future coordinated radio and X-ray observations. Overall, our results show that neutron stars do not follow a single relation between inflow and outflow, and confirm that their accretion dynamics are more complex than for black holes.

==> oldtable.tex <==

\begin{rotatetable}
\begin{deluxetable*}{ccccccll} 
\tabletypesize{\scriptsize}
\tablecaption{Quasi-Simultaneous Radio and X-ray Observations of NSXBs} 
\tablehead{Source & GC & RA & Dec & Radio Date & Flux Density & X-ray Date & Flux Density\\
 & (arcsec) &  & & & (mJy bm$^{-1}$) & & (ergs s$^{-1}$cm$^{-2}$)}
\startdata
4U\,1820$-$30 & NGC\,6624 & 18:23:40.495 & $-$30:21:40.12 & 2014 July 17.21 & $236\pm27.1$ & 2014 July 19.06 & 9.6$^{-9}\pm0.2$ &\\
&&&& 2015 Apr 24.41 & $235\pm5.1$ & 2015 Apr 24.10 & $1.5$^{-9}$\pm0.1$ & \\
4U\,1746$-$37 & NGC\,6441 & 17:50:12.695 & $-$37:03:06.56 & 2015 Apr 14.41 & $<$13.7 & 2015 Apr 13.04 &  $8.6$^{-10}$\pm2$ & \\
XB\,1832$-$330 & NGC\,6652 & 18:35:43.656 & $-$32:59:26.35 & 2017 May 22.03 & $<$6.6 & 2017 May 22.12 & $1.9$^{-11}$\pm0.1$ & \\
X1850--087  & NGC\,6712 & 18:53:04.867 & $-$08:42:20.34 & 2014 Apr 5.08 & $<$12.9 & 2014 Apr 6.07 & $1.6$^{-9}$\pm0.1$ &\\
GRS\,1747$-$312 & Ter\,6 & 17:50:46.860 & $-$31:16:28.88 & 2015 Apr 17.41 & $213\pm5.1$ & 2015 Apr 16.04 & $7$^{-12}$^{+130.0}_{-4.0}$ &\\
&&&& 2018 Mar 26.08 & $<$12.9 & 2018 Mar 26.04 & $4.7$^{-12}$^{+4.9}_{-2.7}$ &\\
&&&& 2018 April 30.08 & $26\pm4.3$ & 2018 May 01.04 & $1.2$^{-12}$^{+1.4}_{-1.0}$ &\\
AC\,211 & M15 & 21:29:58.310 & 12:10:02.66 & 2011 May 30.12 &  $292\pm6.3$ & 2011 May 31.01 & 4.46$^{-10}\pm0.05$ &\\
X-2 & M15 & 21:29:58.132 & 12:10:02.24 & 2011 May 30.12 & $205\pm6.3$ & 2011 May 31.01 & $9.46^{-10}\pm0.034$ & \\
X-3 & M15 &  21:29:58.161 & 12:09:39.93 & 2011 May 30.12 & $<$16.1 & 2011 May 31.01 & $3.5 $^{-13}$ $^{+1.4}_{-0.8}$ \\
\enddata
\label{quasisim}
\tablenotetext{b}{See also \citet{Crawford11}.}
\end{deluxetable*}
\end{rotatetable}

